Lexical Entrainment for Conversational Systems

Conversational agents have become ubiquitous in assisting with daily tasks, and are expected to possess human-like features. One such feature is lexical entrainment (LE), a phenomenon in which speakers in human-human conversations tend to naturally and subconsciously align their lexical choices with those of their interlocutors, leading to more successful and engaging conversations. As an example, if a digital assistant replies 'Your appointment for Jinling Noodle Pub is at 7 pm' to the question 'When is my reservation for Jinling Noodle Bar today?', it may feel as though the assistant is trying to correct the speaker, whereas a response of 'Your reservation for Jinling Noodle Bar is at 7 pm' would likely be perceived as more positive. This highlights the importance of LE in establishing a shared terminology for maximum clarity and reducing ambiguity in conversations. However, we demonstrate in this work that current response generation models do not adequately address this crucial humanlike phenomenon. To address this, we propose a new dataset, named MULTIWOZ-ENTR, and a measure for LE for conversational systems. Additionally, we suggest a way to explicitly integrate LE into conversational systems with two new tasks, a LE extraction task and a LE generation task. We also present two baseline approaches for the LE extraction task, which aim to detect LE expressions from dialogue contexts.

==> paper/rebuttal.tex <==
\section{Author Response to the Area Chair (kjJB)}
We express our sincere gratitude for reviewers’ insightful comments and constructive feedback. We are thrilled to receive positive feedback from the meta-reviewer (kjJB) regarding (1) \textit{the precise definition of the concept}, (2) \textit{the significance of our proposed dataset}, and (3) \textit{our success in highlighting existing challenges in dialogue systems}. We concur with the meta-reviewer's assessment that the concerns raised by the reviewers are largely minor. We are confident that most of the points raised by the reviewers can be comprehensively addressed in the camera-ready version given the extra page of content. 

For the suggestions from the meta-reviewer (kjJB), we are committed to addressing them as follows:
\begin{itemize}
    \item \textbf{Final Agreement Rate}. We agree with reviewer (ZcoZ) and meta-reviewer (kjJB) about the necessity of annotating a new set of 50 dialogues. We will measure a final agreement rate and include this in our revised paper. 
    \item \textbf{Terminology and Definition of Lexical Entrainment}. We acknowledge the meta-reviewer (kjJB)’s recommendation for a broader and more general definition of lexical entrainment, as in previous works \cite{pickering_garrod_2004,reitter-etal-2006-computational}. We will revise our work to incorporate this change in terminology and offer a clearer explanation.
    \item \textbf{Inclusion of Related Works}. We thank the meta-reviewer (kjJB) for pointing out the work of \citet{brockmann2005modelling} and \citet{bakshi-etal-2021-structure}'s papers, which are related to our paper. We will discuss these works in our revised version. 
    \item \textbf{Alternative Measurement using BLEU-2}. We agree with the meta-reviewer (kjJB) that BLEU-2 as an alternative measure for other corpora is a significant suggestion. In our revised paper, we will discuss its potential advantages and also explore its effectiveness against our annotated MultiWOz dataset.
\end{itemize}


==> table/statistics_domains.tex <==
\begin{table}[htbp]
\centering
\scriptsize
\caption{Statistics for train, valid, and test sample for five domains.}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{cccccc}
\hline
\hline
      & Taxi & Hotel & Attraction & Train & Restaurant \\ \hline
Train & 7454 & 14855 & 12273      & 12737 & 15511      \\
Valid & 877  & 1905  & 1801       & 2031  & 1995       \\
Test  & 912  & 1857  & 1902       & 2134  & 2028       \\ \hline \hline
\end{tabular}
\end{adjustbox}
\label{tbl:statistics_wrt_domains}
\end{table}
